Percolation and connection times in multi-scale dynamic networks

We study the effects of mobility on two crucial characteristics in multi-scale dynamic networks: percolation and connection times. Our analysis provides insights into the question, to what extent long-time averages are well-approximated by the expected values of the corresponding quantities, i.e., the percolation and connection probabilities. In particular, we show that in multi-scale models, strong random effects may persist in the limit. Depending on the precise model choice, these may take the form of a spatial birth-death process or a Brownian motion. Despite the variety of structures that appear in the limit, we show that they can be tackled in a common framework with the potential to be applicable more generally in order to identify limits in dynamic spatial network models going beyond the examples considered in the present work.

==> custDefs.tex <==
\def\Spec{\ms{Spec}}
\def\A{\mathbb A}
\def\lan{\langle}
\def\ran{\rangle}
\def\K{\underline{K}}
\def\wt{\widetilde}
\def\H{\text{H}}
\def\wh{\widehat}
\def\udot{\mathaccent\cdot\cup}
\def\coloneqq{:=}
%\def\G{\mathbb G}
\def\ldot{.}
\def\Inv{\ms{Inv}}
\def\KM{K^\ms{M}_*/2}
\def\KMk{K^\ms{M}_*(k_0)/2}
\def\KW{\KM}
\renewcommand\k{\kappa}
\def\k{\kappa}
\def\OO{\ms O}
\def\Oc{\mc O}
\def\tot{\ms{tot}}
\def\charr{\ms{char}}
\def\res{\ms{res}}
\def\e{\varepsilon}
\def\de{\delta}
\def\a{\alpha}
\def\b{\beta}
\def\Gal{\ms{Gal}}
\def\dec{\ms{dec}}
\def\fmil{f^{\ms{Mil}}}
\def\wda{W(D_6) \times \langle s_{a_4}\rangle}
\def\T{\mathbb{T}}

\def\Ab{\mc Ab}
\def\Fk{\mc F_{k_0}}
%\def\Sm{\mc Sm}

\makeatletter
\newcommand{\addresseshere}{%
  \enddoc@text\let\enddoc@text\relax
}
\makeatother

\def\Vsg{V^{\star\Gamma}}
\def\mi{\mf I}
\def\mt{\mf T}
\def\mp{\mf P}
\def\mz{\mf Z}
\def\Vi{V(\mi)}
\def\hes{\hat E_s}
\def\sma{S_n^{M,\alpha}}
\def\sa{S_n^{\alpha}}


